Unicron: Economizing Self-Healing LLM Training at Scale

Training large-scale language models is increasingly critical in various domains, but it is hindered by frequent failures, leading to significant time and economic costs. Current failure recovery methods in cloud-based settings inadequately address the diverse and complex scenarios that arise, focusing narrowly on erasing downtime for individual tasks without considering the overall cost impact on a cluster. We introduce Unicron, a workload manager designed for efficient self-healing in large-scale language model training. Unicron optimizes the training process by minimizing failure-related costs across multiple concurrent tasks within a cluster. Its key features include in-band error detection for real-time error identification without extra overhead, a dynamic cost-aware plan generation mechanism for optimal reconfiguration, and an efficient transition strategy to reduce downtime during state changes. Deployed on a 128-GPU distributed cluster, Unicron demonstrates up to a 1.9x improvement in training efficiency over state-of-the-art methods, significantly reducing failure recovery costs and enhancing the reliability of large-scale language model training.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all: paper

paper: paper.pdf
.PHONY: paper

paper.pdf:
	pdflatex -interaction=nonstopmode paper.tex || true
	- bibtex paper.aux
	pdflatex -interaction=nonstopmode paper.tex || true
	pdflatex -interaction=nonstopmode paper.tex
.PHONY: paper.pdf

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux *.fdb_latexmk \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \



clean: docclean
	# $(RM)  $(PACKAGE).cls 
	

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> sec-related.tex <==
\section{Related Work}
\label{sec:related}

\stitle{Failure Detection in Training.} Cloud providers like AWS and Alibaba cloud have provided operation and maintenance tools for users to monitor the status of clusters and locate faulty nodes.
However, these tools only offer coarse-grained monitoring and are not designed for the training process.
Recent works such as GEMINI~\cite{wang2023gemini} and TRANSOM~\cite{wu2023transom} aim to detect failures more quickly and accurately by introducing monitoring agents that check the GPU status and logs. 
These works differ from \spk, as they typically rely on out-of-band monitoring.
Instead, \spk~provides fine-grained error detection per critical step on each GPU through in-band monitoring inserted into the communication module in the training framework, which is more accurate and efficient.

\stitle{Checkpointing in Training.} Major deep learning frameworks like PyTorch~\cite{li2020pytorch} and TensorFlow~\cite{abadi2016tensorflow} have provided checkpointing mechanisms for users to save models and data during the training process.
Several studies have also focused on optimizing the checkpointing mechanism for model training scenarios~\cite{wang2023gemini, mohan2021checkfreq, eisenman2022check, nicolae2020deepfreeze}.
Recognizing the necessity of checkpointing for failure recovery as a bottom-up solution, \spk~also adopts the checkpointing mechanism. 
Our work is orthogonal to these studies as we focus on the top-down solution.
More optimized checkpointing mechanisms can be integrated into \spk~to further reduce the overhead incurred by interrupted stages.

\stitle{Elastic Training/Scheduling.} Some works~\cite{KungFu, Elastic, 9373916, Elan, Lyra, shukla2022singularity} propose methods to enable elastic training/scheduling for distributed model training, but they are not designed for the 3D parallelism architecture.
Oobleck~\cite{jang2023oobleck} is the first work that adopts dynamic reconfiguration to enable resilient distributed training with guaranteed fault tolerance, following the 3D parallelism architecture.
However, it is only designed for utilizing all available resources for a single task, lacking  consideration for multiple training tasks running on the same cluster and the overall economic cost. 
Our cost model in \spk~is designed to address these issues and generate the optimal reconfiguration plan.
Furthermore, the fast transition strategy in \spk~is designed to reduce the overhead of reconfiguration, which is another key improvement compared to existing solutions.


\section{Conclusion}
\label{sec:conclusion}
This paper introduces the \spk~system as a novel solution for overcoming the challenges of failure recovery in large-scale model training on the cloud. 
\spk~takes a global perspective, aiming to minimize the overall cost introduced by failures considering the scenario of multiple training tasks running on the same cluster.
To achieves this goal, \spk~incorporates (1) in-band error detection without causing additional overhead during training, (2) a cost-aware recovery mechanism that dynamically selects the most suitable reconfiguration plan based on various factors, and (3) a fast transition strategy to reduce the duration of reconfiguration.
\spk~significantly reduces the overall cost of failure recovery, achieving savings of up to $xxx\%$ when compared to state-of-the-art solutions.
